Spatiotemporal Data Mining: A Survey on Challenges and Open Problems

Spatiotemporal data mining (STDM) discovers useful patterns from the dynamic interplay between space and time. Several available surveys capture STDM advances and report a wealth of important progress in this field. However, STDM challenges and problems are not thoroughly discussed and presented in articles of their own. We attempt to fill this gap by providing a comprehensive literature survey on state-of-the-art advances in STDM. We describe the challenging issues and their causes and open gaps of multiple STDM directions and aspects. Specifically, we investigate the challenging issues in regards to spatiotemporal relationships, interdisciplinarity, discretisation, and data characteristics. Moreover, we discuss the limitations in the literature and open research problems related to spatiotemporal data representations, modelling and visualisation, and comprehensiveness of approaches. We explain issues related to STDM tasks of classification, clustering, hotspot detection, association and pattern mining, outlier detection, visualisation, visual analytics, and computer vision tasks. We also highlight STDM issues related to multiple applications including crime and public safety, traffic and transportation, earth and environment monitoring, epidemiology, social media, and Internet of Things.

==> Response.tex <==
\section*{Response}
We would like to extend our appreciation for the comments of the reviewers. The comments helped improve the quality and readability of the revised manuscript. Kindly find below our replies to the comments. \textcolor{blue}{The replies are coloured in blue} and the \textcolor{red}{changes made in the article are in red colour}.
Also, we have extended the survey to cover \textcolor{darkgreen}{recent studies in new topics, coloured in green}.

\section*{General note:}
In this edited version, we added new paragraphs and figures to the introduction to highlight motivations and describe STDM. We extended the big data and cloud computing section to review the spatial cloud computing.
We have added a new section 3.5.5 Fairness, Accountability, Transparency, and Ethics (FATE). Besides, we have extended the following sections to cover bias, fairness, and explainability topics in STDM:
\begin{itemize}
    \item 3.4.4 Social
    \item 4.1 Spatiotemporal Prediction
    \item 5.1 Crime and Public Safety 
    \item 5.2 Traffic and Transportation
    \item 5.3 Earth and Environment Monitoring
    \item 5.6 Smart Internet of Things
\end{itemize}
We have also updated other sections to cite recent works in spatiotemporal representation, advanced modelling, and visualisation. Moreover, figures across the paper are also redesigned and updated.

% \begin{itemize}
%     \item 3.4.4 Social $\leftarrow$ Bias in Machine Learning algorithms such as in face recognition and employee hiring.
%     \item 4.1 Spatiotemporal Prediction $\leftarrow$ Model explainability. 
%     \item 5.1 Crime and Public Safety $\leftarrow$ Bias in predictive policing. 
%     \item 5.2 Traffic and Transportation $\leftarrow$ Fairness in ride-hailing platforms. 
%     \item 5.3 Earth and Environment Monitoring $\leftarrow$ Bias correction in climate forecast  and commercial vessel traffic.
%     \item 5.6 Smart Internet of Things $\leftarrow$ Bias correction in multiple sensor data fusion.
% \end{itemize}

The current content is extended and the total word count is increased from \textbf{9,693} to
\textbf{11,601}.
% \textbf{11,556}.
% \textbf{11,262}.
% \textbf{10,975}.
% \textbf{10,244}.
We have updated the bibliography with the new publications in the artificial intelligence and pattern recognition venues. The bibliography references have increased form \textbf{288} to \textbf{342}.

\section*{Reviewer \#3}
All my comments are addressed, would suggest to add a review on spatial cloud computing, which is cloud computing for spatiotemporal data. Congratulations to the authors!
\newline
\textcolor{blue}{We extended  the big data and cloud computing section (3.4.9) to include spatial cloud computing as follows:}
\newline
\textcolor{red}{Specifically, conventional cloud computing techniques are not designed to handle the spatiotemporal data. Therefore, spacial cloud computing techniques have recently been proposed to leverage a layer of data-as-a-service (DaaS) to virtualise the spatiotemporal data \cite{yang2011spatial}. 
The advancements of the GIS harnessed the wide availability of the cloud-based spatiotemporal services \cite{qingquan2014big}. Spatiotemporal data storage and parallel processing are widely provided by open-source cloud systems \cite{yao2018landqv2}. Other technologies such as Esri Geospatial Cloud and Google Earth Engine are also providing significant Earth observations spatiotemporal data. Overall, spatial cloud computing aims to solve spatiotemporal issues related to storage and processing. It also tends to offer better spatiotemporal data utilisation through the "as-a-service" paradigm. However, there is a difficulty in representing physical spatiotemporal phenomena that are continuous via the classical discrete based cloud approaches. This issue stems from the heterogeneity, dynamic scalability, and complex distributions of the spatiotemporal data.
}
\section*{Reviewer \#4}
The paper reviews the challenges and open problems in STDM. The challenges are categorized in 3 perspectives from general to specific tasks/applications. The table at the end of the paper summarizes the challenges together with related works attempting to address them which is helpful to researchers. 
However, it suffers from several nontrivial issues before it is ready to be published.
\newline
\begin{enumerate}
    \item Lack of background: \newline
    The paper first briefly introduces what is spatiotemporal data and then directly goes to the challenges of STDM, without necessary introduction on what is STDM and why it is important. It would be helpful to a section containing 
    basic concepts of spatiotemporal data mining %%% 
    before heading into the analysis of the issues.
    \newline
    \textcolor{blue}{We updated the introduction section to provide background information on STDM including definitions, and research motivations and significance.
    We explained the spatiotemporal data types from discrete and continuous measuring perspectives. We added illustrative figures for the correspondent data types. Besides, we highlighted the utilisation of STDM in different applications and scales. We explained some issues of classical data mining techniques that led to the need for STDM development. The text in Section 1 is updated as follows:
    }
    \newline
    \newline
\textcolor{red}{
Large amounts of spatiotemporal data are being generated and captured through systems that record sequential observations of remote sensing, mobility, wearable devices, and social media. Spatiotemporal data represent different phenomena ranging from micro-scale of DNA and cell evolution, to global ones, e.g., climate change \cite{Chaowei2019Big}. The wide-availability of user-generated data via the social media platforms offers great opportunities to understand people needs, thoughts, and sentiments toward specific topics, products, or services \cite{Hamdi2018CLASENTI}. Medical sensory devices observe different activities at various locations of the human body over specific time ranges.
%
STDM proposes new methods to handle such data through advanced predictive and descriptive tasks such as classification and clustering to work best with space and time referenced data. 
STDM methods are concerned with relationships and dependencies among different measurements. These relationships are complex, implicit, and dynamically changing.
To a large extent, classical data mining assumes that data are independent and identically distributed (i.i.d.). On the contrast, spatiotemporal data do not follow this assumption and STDM methods aim to capture the autocorrelation among different events or data points that are interdisciplinary in nature, i.e, data from multiple domains that may require the utilisation of various mining tasks.
%
\newline
\newline
Spatiotemporal data comprise spatial and temporal representations. They include three distinct types of attributes, namely, non-spatiotemporal, spatial and temporal attributes \cite{RN14t}. The non-spatiotemporal attributes represent non-contextual features of objects. Spatial attributes define the locations, extents, and shapes of the objects. Temporal attributes are timestamps and durations of processes denoting spatial object (vector) or field (raster layers). For example, air pollution spatiotemporal data have non-spatiotemporal attributes such as air pollution levels or station names, spatial coordinates of the location where the measurements are taken and temporal timestamps associated with the collected measurements.
Spatiotemporal data types can also be categorised based on their collection nature to discrete or continuous observations. Events and data trajectories are examples of spatiotemporal discrete data types, while continuous data types include point reference and raster data.
Spatiotemporal event data constitute discrete events that happen at geo-locations and times such as traffic accidents and crime incidents. Figure \ref{ST_types} (a) denotes spatiotemporal events of three different types. Each type is presented in different colour and shape, e.g., red circles are for events of one type and each event is annotated with the its location and time (location $l_1$ in time $t_1$).
Trajectory data contain sequences of spatiotemporal instances that trace motions of objects in geographical spaces overtimes. Trajectories are usually represented by a series of chronologically ordered points which consist of spatial coordinates and timestamps \cite{zheng2015trajectory}. For instance, a vehicle trajectory between two locations is a set of consecutive points of space and time. Figure \ref{ST_types} (b) illustrates trajectories of three coloured objects between locations ($l_1$ and $l_n$) at times ($t_1$ and $t_2$). 
Point reference data measure continuous spatiotemporal fields at moving spatiotemporal reference sites. For example, spatiotemporal point references can be utilised to measure surface temperature using moving balloons. Figure \ref{ST_types} (c and d) show spatiotemporal point reference data at different locations (black squares) at timestamps ($t_1$ and $t_2$).
Raster data represent measurements of spatiotemporal fields at fixed cells in  grids such as activities in fMRI brain scans. Figure \ref{ST_types} (e and f) show spatiotemporal raster data of regular grid at time ($t_1$ and $t_2$).
These different types of spatiotemporal data are associated with different research challenges \cite{RN357}. Classical data mining approaches are not designed to handle such data. 
%
\begin{figure}[]%[bt]
\centering
\includegraphics[width=0.99\textwidth, angle=0]{ST-Data-2.jpg}
\caption{\textcolor{red}{Spatiotemporal data types. (a) spatiotemporal events of different types at different locations and timestamps. (b) spatiotemporal trajectories between locations ($l_1$ and $l_n$) at time ($t_1$ and $t_2$). (c and d) spatiotemporal point reference data at different locations at timestamps ($t_1$ and $t_2$). (e and f) spatiotemporal raster data of regular grid at time ($t_1$ and $t_2$).}}
\label{ST_types}
\end{figure}
}
    \newline
    \item Readability
    \begin{enumerate}[label=(\alph*)]
        \item The paper contains numerous grammar mistakes and typos. To mention a few,
        \begin{enumerate}[label=(\roman*)]
            \item "We attempt to fill this gap providing a comprehensive literature survey on state-of-the-art advances in STDM." providing -$>$ by providing 
            \textcolor{blue}{$\leftarrow$ Corrected}.
            \textcolor{red}{We attempt to fill this gap by providing a comprehensive literature survey on state-of-the-art advances in STDM.}
            \item "It includes three distinct types of attributes, namely; non-spatiotemporal, spatial and temporal attributes." Incorrect usage of semicolon 
            \textcolor{blue}{$\leftarrow$ Corrected}.
            \textcolor{red}{It includes three distinct types of attributes, namely, non-spatiotemporal, spatial and temporal attributes \cite{RN14t}.}
            \item "the pattern of a moving object might be affected by nearby objects such as a car direction, speed and acceleration are influenced by other cars around it." car -$>$ car's 
            \textcolor{blue}{$\leftarrow$ Corrected}.
            \textcolor{red}{In other words, the pattern of a moving object might be affected by nearby objects such as a car's direction, speed and acceleration are influenced by other cars around it.} 
            \item "each of which discussed the literature form different perspective such as spatial databases" form -$>$ from, perspective -$>$ perspectives 
            \textcolor{blue}{$\leftarrow$ Corrected}.
            \textcolor{red}{There have been several survey articles that reviewed work related to STDM, each of which discussed the literature from different perspectives such as spatial databases \cite{koperski1996spatial}, spatial patterns \cite{RN172}, spatiotemporal cluster analysis \cite{RN173}, urban concepts and applications \cite{Zheng2014Urban}, big data analytics \cite{yang2019big}, big climate data analytics \cite{hu2018climatespark}, and outliers detection \cite{RN174,meng2018overview}.}
            \item "Visualisations in data analysis are important for the decision-making as they visually summarise and present results indigestible and easy to understand forms." Indigestible -$>$ in digestible each of which discussed the literature
            \textcolor{blue}{$\leftarrow$ Corrected}.
            \textcolor{red}{Visualisations in data analysis are important for the decision-making as they visually summarise and present results in digestible and easy to understand forms.} 
        \end{enumerate}
    \item The paper contains incomprehensible sentences.
    \begin{enumerate}[label=(\roman*)]
        \item "The spatial and temporal correlation among the traffic variables led there modelling to better results." 
        \textcolor{blue}{$\leftarrow$ Corrected}.
        \textcolor{red}{The spatial and temporal correlation among the traffic variables led to better results.}
        \item "The latter aggregates the sensing data, which leads to loss of data about tracking the relationships between them." 
        \textcolor{blue}{$\leftarrow$ Corrected}.
        \textcolor{red}{The latter aggregates the sensing data. This data aggregations leads to loss of data about tracking the relationships between them.}
    \end{enumerate}
    \end{enumerate}
\end{enumerate}



